Improving robustness of spontaneous speech synthesis with linguistic speech regularization and pseudo-filled-pause insertion

We present a training method with linguistic speech regularization that improves the robustness of spontaneous speech synthesis methods with filled pause (FP) insertion. Spontaneous speech synthesis is aimed at producing speech with human-like disfluencies, such as FPs. Because modeling the complex data distribution of spontaneous speech with a rich FP vocabulary is challenging, the quality of FP-inserted synthetic speech is often limited. To address this issue, we present a method for synthesizing spontaneous speech that improves robustness to diverse FP insertions. Regularization is used to stabilize the synthesis of the linguistic speech (i.e., non-FP) elements. To further improve robustness to diverse FP insertions, it utilizes pseudo-FPs sampled using an FP word prediction model as well as ground-truth FPs. Our experiments demonstrated that the proposed method improves the naturalness of synthetic speech with ground-truth and predicted FPs by 0.24 and 0.26, respectively.

==> tab/eval_notused_1.tex <==
\begin{table}[t]
\vspace{-2mm}
\caption{Preference scores of consistency training with pseudo-FPs sampled using FP prediction model with various loss ratios ($\beta$).}
\vspace{-3mm}
\label{tab:eval3}
\begin{center}
\footnotesize
\begin{tabular}{c|ll|l}
\hline
$\beta$ & \multicolumn{1}{c}{Score} & \multicolumn{1}{c|}{p-value} & $\beta$ \\ \hline
1.0    & 0.457 vs. \textbf{0.543}  & $3.38\times10^{-2}$          & 2.0    \\
2.0    & 0.400 vs. \textbf{0.600}  & $7.86\times10^{-7}$          & 4.0    \\ \hline
\end{tabular}
\end{center}
\vspace{-6mm}
\end{table}

==> tab/mos_notused.tex <==
\begin{table}[t]
\vspace{-2mm}
\caption{Mean opinion scores of synthetic speech with FPs by the baseline model (i.e., trained without consistency loss) and the best-proposed model (i.e., trained with consistency loss for probabilistically sampled FPs with $\alpha=1.0$ and $\beta=4.0$).}
\vspace{-3mm}
\label{tab:mos}
\begin{center}
\footnotesize
\begin{tabular}{c|c|c}
\hline
Method                                                                          & Utterance & Mean ± 95\% conf interval \\ \hline
\multirow{2}{*}{Baseline}                                                          & TrueFP    & 3.350 ± 0.125             \\
                                                                                & PredFP    & 3.280 ± 0.125             \\ \hline
\multirow{2}{*}{Proposed} & TrueFP    & 3.590 ± 0.121             \\
                                                                                & PredFP    & 3.537 ± 0.117             \\ \hline
\end{tabular}
\end{center}
\vspace{-4mm}
\end{table}
